Multi-Granularity Video Object Segmentation

Current benchmarks for video segmentation are limited to annotating only salient objects (i.e., foreground instances). Despite their impressive architectural designs, previous works trained on these benchmarks have struggled to adapt to real-world scenarios. Thus, developing a new video segmentation dataset aimed at tracking multi-granularity segmentation target in the video scene is necessary. In this work, we aim to generate multi-granularity video segmentation dataset that is annotated for both salient and non-salient masks. To achieve this, we propose a large-scale, densely annotated multi-granularity video object segmentation (MUG-VOS) dataset that includes various types and granularities of mask annotations. We automatically collected a training set that assists in tracking both salient and non-salient objects, and we also curated a human-annotated test set for reliable evaluation. In addition, we present memory-based mask propagation model (MMPM), trained and evaluated on MUG-VOS dataset, which leads to the best performance among the existing video object segmentation methods and Segment SAM-based video segmentation methods. Project page is available at https://cvlab-kaist.github.io/MUG-VOS.

==> AnonymousSubmission/Writing/3_Task.tex <==
\section{Video segment anything}
\subsection{Video segment anything task}
Traditional video segmentation tasks~\cite{Shaker2024MAVOS, su2023motion} aim to segment targets such as objects or target semantics according to specific purposes. These tasks are useful in applications where the targets to be segmented are clearly defined, but they have limitations when applied to many real-world applications like user interactive video editing~\cite{deng2023dragvideo, huang2023inve, tilekbay2024expressedit}, where the targets are not predetermined. To tackle this issue, we introduce the video segment anything task.

\paragraph{Task format.}
Video segment anything task aims to segment any targets in the video clip from the prompts provided in the initial frame. For a video clip with $T$ frames, images of each frame are sequentially input with the prompts in the initial frame. In this work, we use prompts derived from the initial masks according to each method. Then we define the annotated mask for each frame identified by each initial prompt set as the target to be predicted. Here, the target includes various types and granularities of objects, stuff, parts, and backgrounds. Therefore, multiple target mask tracks can share the same regions, and we conduct independent evaluations for each target.

\paragraph{Evaluation metric.}
We adopt standard VOS evaluation metrics for evaluating ViSA. Standard VOS evaluation does not allow the intersection of the masks since the VOS metric annotate multiple masks to a single frame. This can not accurately evaluate the variety of masks in a single frame, so we modified it to measure masks in a one-to-one manner. We asses $\mathcal{J} \& \mathcal{F}$ which is average of Jaccard Index~\cite{everingham2010pascal} $(\mathcal{J})$ and boundary F1-score~\cite{perazzi2016benchmark} $(\mathcal{F})$.

==> AnonymousSubmission/Writing/4_Data.tex <==
\input{AnonymousSubmission/figure/latex/visa_engine_figure}


\section{Dataset}
Existing video segmentation datasets~\cite{xu2018youtube, pont20172017, wang2021unidentified, Miao_2022_CVPR, athar2023burst} typically focused on salient target objects that can be defined as specific classes. 
% Since SAM can generate class-agnostic masks based on user prompts, Video Segment Anything should also be capable of segmenting any object and even background clutters in a video scene. 
However, there currently exists no dataset for training or evaluating a diverse granularity of masks in video segmentation task.

Despite the numerous datasets for image-level segmentation, video-level segmentation datasets are scarce. Additionally, the lack of densely annotated masks in current video datasets hinders the adaptation of SAM on video segmentation.
In order to train and evaluate MMPM, a large-scale video segmentation dataset is needed. To satisfy such conditions, Annotating a mask in a handcrafted way is accurate, but costs a lot. 
% Therefore, we present to automatically generate a novel video segmentation dataset. 
Therefore, we employ a semi-automatic data generation process involving minimal human annotators. To create a sufficiently large and diverse dataset, we developed a data collection pipeline to collect video segmentation data with varied granularity masks. Our data collection pipeline produces the segmentation data in a step-wise manner, ensuring both the quality and quantity of the masks. 

\subsection{Data collection pipeline}
% In contrast to the abundance of datasets tailored for image-level segmentation, those dedicated to video-level segmentation are conspicuously rare. Moreover, the prevailing deficiency in densely annotated masks within existing video datasets presents formidable obstacles to the adaptation of SAM for video segmentation, impeding advancements in research within this domain. To mitigate these constraints, 
We propose a data collection pipeline designed to autonomously derive video segmentation data from pre-existing video sources. Our data collection pipeline exploits SAM to generate dense masks for each frame and leverages an optical flow model to establish temporal connections between masks across consecutive frames, thereby generating pseudo-masks for video segmentation.

More specifically, for the given video \(V=\{v_t\vert t\in [1,T]\}\), where \(v_t\) is $t$-th frame image, and \(T\) is the number of frames, target masks \(M_t^i\) are defined as those obtained from the initial frame using SAM through grid point prompts. Masks from subsequent frames that are temporally consistent to the masks from the initial frame, where \(i\) is the index of the track containing the target masks. Following the initial frame, prior to obtaining the target mask in the \(t\)-th frame, candidate masks potentially serving as the target mask are predicted. 

To generate the candidate masks \(C_t^i\), the points \(P_t^i\) are sampled from the target mask \(M_{t-1}^i\). Subsequently, the points \(W_t^i\) are derived by warping the sampled points \(P_t^i\) into the \(t\)-th frame utilizing a flow map \(F_{t-1 \rightarrow t}\) predicted by a flow model.
\begin{equation}
    P_t^i = \mathrm{sample}(M_{t-1}^i) \\
\end{equation}
\begin{equation}
    W_t^i = \mathrm{warp}(P_t^i, F_{t-1\rightarrow t})
\end{equation}
\begin{equation}
    F_{t-1\rightarrow t} = \mathrm{flow}(v_{t-1}, v_t)
\end{equation}
The \(\mathrm{sample}\) function denotes the process of randomly selecting point coordinates on the mask, while the \(\mathrm{warp}\) function represents the warping of a point or a mask according to the flow map. The \(\mathrm{flow}\) function refers to the estimation of a flow map between two adjacent frames.
Candidate masks \(C_t^i\) in the \(t\)-th frame are derived by applying the point prompts acquired from the warped points \(W_t^i\) to SAM. The target mask \(M_{t-1}^i\) is further warped to the \(t\)-th frame via the flow map \(F_{t-1\rightarrow t}\) to obtain the warped mask \(\tilde{M}_{t-1}^i\). Subsequently, the Intersection over Union (IoU) between the warped mask \(\tilde{M}_{t-1}^i\) and the candidate masks \(C_t^i\) are computed, with the candidate mask exhibiting the highest IoU being designated as the target mask \(M_t^i\) in the \(t\)-th frame.
\begin{equation}
    C_t^i = \mathrm{SAM}(v_t, W_t^i)
\end{equation}
\begin{equation}
    \tilde{M}_{t-1}^i = \mathrm{warp}(M_{t-1}^i, F_{t-1\rightarrow t})
\end{equation}
\begin{equation}
\label{iou_eq}
    M_t^i = \arg\max_{C_t^i}\mathrm{IoU}(\tilde{M}_{t-1}^i, C_t^i)
\end{equation}
% Only mask tracks with an Intersection over Union (IoU) exceeding a threshold \(\gamma\) are included in the final dataset for all frames \(t\).

\paragraph{Quality assurance.}
Fully automated processes can induce significant errors in the evaluation procedure. To prevent errors from accumulating in the automated process, human annotators were tasked with manually tracking and generating masks. For efficiency, annotators were instructed to accept or reject the mask tracks produced by the data collection pipeline. If an error occurred, the annotators refined the mask at the frame level using SAM. More details can be found in the appendix.

To ensure the quality of the mask tracks in the dataset, we adopted a verification process. As human annotators conduct the tracking process, completed tracks are sent to a supervisor for approval. The supervisor reviews the annotated mask tracks alongside the original video to determine whether the tracks are satisfactory or unsatisfactory. Rejected mask tracks are sent back to the annotators for refinement.
Quality assurance process was only done on the MUG-VOS test dataset.

\subsection{MUG-VOS Dataset}
The MUG-VOS dataset was built using our data collection pipeline and, to the best of our knowledge, is larger than any other video segmentation dataset.

\paragraph{Video collection.}
In the pursuit of crafting the video segmentation dataset, a judiciously selected subset of videos from the HD-VILA-100M~\cite{xue2022hdvila} dataset was scrupulously curated for inclusion. The HD-VILA-100M dataset is devised to function as an expansive, high-resolution, and diversified video-language dataset, with the overarching goal of fostering multi-modal representation learning. This dataset encompasses a total of 3.3 M videos, characterized by their high caliber and equitable distribution across 15 categories. A subset of videos from this dataset was processed to get 77,994 video clips.

In addition, We create additional annotations for the 30 videos in the DAVIS-17\cite{pont20172017} validation set, which widely used in VOS task, for MUG-VOS test sets. We use SAM to generate average 29.6 mask tracks of varying types and granularities for each video.
% To generate consistent masks for each video, we use our proposed SAM-based annotation tool. 

\paragraph{Data generation.}
The MUG-VOS dataset facilitates training and evaluation on masks with various types and granularities, which are not covered by existing video segmentation datasets. Our data collection pipeline simplifies this process while ensuring high quality. To achieve this, we adapted our pipeline to the HD-VILA-100M and DAVIS-17 videos, resulting in a dataset that is both high quality and large in scale.
% Therefore, we propose a method of generating large-scale training datasets via automated annotation of extensive videos to train models for our task.

% We construct our video segmentation dataset using SAM and IoU-based tracking methods. For this, we first collect large-scale, high-resolution, and diversified video data from the video-language dataset HD-VILA-100M~\cite{xue2022advancing}, and create dense masks about each frame using SAM. We connect masks created in each frame using an IoU-based tracking method.


\paragraph{Data statistics.}
\input{AnonymousSubmission/table/data_stat}
Table~\ref{Table:statistics} presents the evaluation of related datasets and benchmarks for video segmentation. The density \( D \) of the segmentation masks is notated in Table~\ref{Table:statistics} can be given by the equation~\ref{eq:density}:
\begin{equation}
\label{eq:density}
    D = \frac{\sum_{i=1}^{H} \sum_{j=1}^{W} M_{i,j}}{H \times W} \\    
\end{equation}
where as \( H \) is the height of the image, \( W \) is the width of the image, \( M_{i,j} \) is the value of the mask at pixel \((i,j)\), which is 1 if the pixel is covered by any mask and 0 otherwise.

For VOS tasks, common benchmarks include YouTube-VOS~\cite{xu2018youtube} and DAVIS~\cite{pont20172017}. Both datasets are annotated on in-the-wild videos, each lasting approximately 5-10 seconds. However, these datasets contain only a few mask tracks per video, which limits their ability to evaluate tracking performance across diverse masks.

The UVO~\cite{wang2021unidentified} dataset primarily focuses on evaluating performance on unseen mask classes during training. It provides mask annotations for a variety of salient objects that humans typically recognize as ``objects''. While UVO covers a wide range of masks from a human perspective, it does not include non-salient objects that are not easily defined by humans, which remains as a limitation.

VIPSeg~\cite{Miao_2022_CVPR} is part of the video panoptic segmentation benchmark. Video panoptic segmentation aims to predict the semantic class of every pixel in the temporal dimension. Compared to the datasets in Table~\ref{Table:statistics}, VIPSeg covers a higher density of pixels than any other dataset in Table~\ref{Table:statistics}. However, the masks in VIPSeg are much simpler compared to MUG, as the number of masks per frame is significantly lower than in MUG.

BURST~\cite{athar2023burst} is a universal dataset designed to cover multiple segmentation tasks, including video object segmentation, video instance segmentation, and point-guided segmentation~\cite{guo2024vanishing, zulfikar2024point}.
While the aforementioned datasets primarily focus on annotating salient objects (e.g., humans, cars, animals), MUG-VOS includes a diverse range of class-agnostic masks.

==> AnonymousSubmission/Writing/5_Model.tex <==
\input{AnonymousSubmission/figure/latex/figure_main}

\section{Model}

\subsection{Preliminaries: revisiting SAM}
SAM consists of an image encoder, prompt encoder, and mask decoder. The input image and the proposed prompts are encoded by the image encoder and the prompt encoder to their embedding space, respectively. The mask decoder receives the image embedding $\mathcal{I}$ and prompt embedding ${p}$, and aggregates them using its two-way transformer to create segmentation masks about the input image and proposed prompts. 

\begin{equation}
    \hat{m}, \hat{p}, \hat{\mathcal{I}} = \mathrm{Trans}(\big[{m}, {p}\big], \mathcal{I}),
\end{equation}

where ${m}$ is the mask embedding, $\mathrm{Trans}(\cdot, \cdot)$ is the two-way transformer block and $\big[\cdot, \cdot\big]$ denotes the concatenation. Since the two-way transformer block aggregate concatenated multi-level mask and prompt embedding with image embedding, SAM can segment any granularity. Note that $\hat{m} \in \mathbb{R}^{n_m \times d}$, $\hat{p} \in \mathbb{R}^{n_p \times d}$, and $\hat{\mathcal{I}} \in \mathbb{R}^{(h \times w) \times d}$ are aggregated output mask embedding, prompt embedding, and image embedding, respectively. Two-way transformer has the token to image attention layers and the image to token attention layers. Token to image attention layer use image embedding as key and value, and prompt embedding as query. Conversely, in the image-to-token attention layer, this relationship is reversed. This architecture allows the image embedding and prompt embedding to learn from each other to generate masks corresponding to both.

\begin{equation}
m^{\text{sa}}, p^{\text{sa}} = \mathrm{Self.Attn}(Q=\big[{m}, {p}\big], ~K=\big[{m}, {p}\big], ~V=\big[{m}, {p}\big]),
\end{equation}
\begin{equation}
m^{\text{ti}}, p^{\text{ti}} = \mathrm{T2I.Attn}(Q=\big[{m}, {p}\big], ~K=\mathcal{I}, ~V=\mathcal{I}),
\end{equation}
\begin{equation}
\hat{\mathcal{I}} = \mathrm{I2T.Attn}(Q=\mathcal{I}, ~K=\big[m^{\text{ti}}, p^{\text{ti}}\big], ~V=\big[m^{\text{ti}}, p^{\text{ti}}\big]),
\end{equation}
\begin{equation}
\hat{m}, \hat{p} = \mathrm{T2I.Attn}(Q=\big[m^{\text{ti}}, p^{\text{ti}}\big], ~K=\hat{\mathcal{I}}, ~V=\hat{\mathcal{I}}),
\end{equation}
where $\mathrm{Attn}$ denotes attention layer that represented as:
\begin{equation}
\mathrm{Attn}(Q,K,V) = \mathrm{Softmax}(\frac{QK^T}{\sqrt{d}})V.
\end{equation}
Finally, the target mask score $\mathcal{M} \in \mathbb{R}^{(h \times w) \times n_m}$ is predicted through the correlation of $\hat{\mathcal{I}}$ and
$\hat{m}$.
\begin{equation}
\mathcal{M} = \hat{\mathcal{I}} \cdot \hat{m}
\end{equation}
In ViSAM, we use SAM with an additional module named prompt generator to transfer to the video domain. The overview of ViSAM is shown in Fig.~\ref{fig:overview}.

\subsection{ViSAM}

To use SAM in the video domain, we introduce the SAM-based video segmentation model ViSAM. To utilize the knowledge of pre-trained SAM, we use the frozen SAM image encoder and prompt encoder, and retrain the two-way transformer of the mask decoder. Additionally, we propose the prompt generator to create dynamic prompts propagated from the previous prompt. Using the prompt generator, we can segment the consistent mask tracks across multi-frames from the provided single-frame prompts. The prompt generator takes the previous output prompt embedding $\hat{p}_{t-1}$ and image embedding of current frame $\mathcal{I}_t$ and outputs the prompt embedding of current frame $p_t$.
\begin{equation}
    {p}_t = \mathrm{PG}(\hat{p}_{t-1}, \mathcal{I}_t),
\end{equation}
where $t$ is the index of each frame and $\mathrm{PG}(\cdot, \cdot)$ denotes the prompt generator module. The prompt generator consists of simple two single-head attention layers.
\begin{equation}
    \hat{p}^{\text{sa}}_{t-1} = \mathrm{Self.Attn}(Q=\hat{p}_{t-1}, ~K=\hat{p}_{t-1}, ~V=\hat{p}_{t-1}),
\end{equation}
\begin{equation}
    p_t = \mathrm{Cross.Attn}(Q=\hat{p}^{\text{sa}}_{t-1}, ~K=\mathcal{I}_t, ~V=\mathcal{I}_t),
\end{equation}
The subsequent process proceeds similarly to SAM. The prompt embedding $p_t$, mask embedding $m$, and image embedding $\mathcal{I}_t$ are input into the mask decoder of SAM.
\begin{equation}
    \hat{m}_t, \hat{p}_t, \hat{\mathcal{I}_t} = \mathrm{Trans}(\big[{m}_t, {p}_t\big], \mathcal{I}_t),
\end{equation}
Subsequently, $\hat{\mathcal{I}_t}$ and $\hat{m}_t$ are correlated to predict the target mask score of the current frame.
\begin{equation}
\mathcal{M}_t = \hat{\mathcal{I}}_t \cdot \hat{m}_t
\end{equation}
The predicted mask score ${M}_t \in \mathbb{R}^{(h \times w) \times n_m}$ supervised with the linear combination of focal loss~\cite{lin2017focal} and dice loss~\cite{milletari2016v} follow \cite{kirillov2023segment}. To conclude, the two-way transformer of the mask decoder and prompt generator learns the context and the consistency from sequentially incoming video data.
\paragraph{Inference}
Due to ViSAM is trained on short video clips, it is unstable when it processes recurrently over the long video data. Hence, in inference time, we additionally use a simple IoU-based tracking method with ViSAM to improve stability. Specifically, we periodically resample the initial prompts from the current predicted mask. In a stable situation where the IoU between the previously predicted mask and the currently predicted mask is greater than the stability constant $\alpha$, we resample the initial prompt $P_t$ that can predict the mask similar to the currently predicted mask. The movement of the target is dynamic, the generated prompts are used recurrently to predict the mask track in subsequent frames.

==> AnonymousSubmission/Writing/5_Model_new.tex <==
\input{AnonymousSubmission/figure/latex/figure_main}

\section{Model}
Figure~\ref{fig:overview} shows the overview of MMPM. For simplicity, the figure assumes a single object, but the MMPM model is designed to handle multiple objects simultaneously. MMPM consistently tracks objects and generates segmentation masks sequentially, frame-by-frame. Thanks to the memory module, which is designed to handle occlusion, motion blur, and deformation, the model can effectively track objects even in challenging video scenes.
To build a robust video segmentation model, we incorporated two types of memory modules that function independently. For each frame, the RGB image is encoded by an image encoder, which serves as a query for the memory module. The encoded query from the image encoder accesses the memory bank to retrieve memory features that provide crucial information for generating the current mask. MMPM uses two types of memory: sequential memory and temporal memory, both of which are updated for selected frame. Frames selected for memory update are selected at regular intervals. Specifically, the temporal memory has a storage limit, $T_{max}$ , to prevent running out of memory. When the temporal memory reaches a store limit, we randomly filter out memory entries, except for those from the first and previous frames. These memory features works as a enhancement for image feature to generate high-quality masks, even in long videos.

\subsection{Temporal memory}
The temporal memory stores information about previous predictions for the same target object in the video by maintaining high-resolution features for up to $T_{max}$ recent frames. We split the memory into key and value components, which effectively retrieve relevant information. The key is encoded in the same embedding space as the query feature, while the value is encoded from a value encoder that fuses semantic and spatial information by encoding the image and binary mask together. Specifically, the key $\mathbb{R}^{C^{k}\times THW}$ exists in the same embedding space as the query feature, while the value is encoded independently.

For a selected frame, we copy the query feature from the image encoder as a key for the current frame. The generated key is then processed along with the binary mask from the mask decoder through the value encoder. The new key and value from the current frame are then appended to the memory and provide important information for future decoding processes. When the number of temporal values reaches $T_{max}$, we randomly sample values, excluding those from the first and previous frames. The first frame's value provides initial information about the target object in the VOS task and is considered to best represent the target object. The value from the last frame contains the latest information about the target object.

This dynamic filtering of the temporal memory enables the model to represent both short-term and long-term object motion effectively.

\subsection{Sequential memory}
While temporal memory focuses on high-resolution features from previous frames, sequential memory focuses on low-resolution features such as geometric, semantic, and location information. Sequential memory complements temporal memory by updating the value on selected frame.

Specifically, sequential memory $S\in\mathbb{R}^{C^{s}\times HW}$ is updated every select frame using the query from the current frame. To effectively propagate sequential information, we use the GRU~\cite{cho2014properties} method, which dynamically forgets previous information and updates with the current frame's information. The output from the value encoder serves as a candidate for updating the sequential memory. The GRU discards outdated information from the previous sequential memory and updates the sequential memory in parallel. This propagation process compensates for the lack of object information in temporal memory and stores new low-resolution information.

\input{AnonymousSubmission/figure/latex/quality_comparison}

% \subsection{Implementation details}
% To fully utilize SAM's pretrained knowledge in the MMPM model, we adopt the ViT-B architecture for the image encoder. The value encoder, which is the core of MMPM, also uses the ViT-B model trained on the SA-1B dataset. To handle the additional channel for the binary mask, we pad the orthogonal weight matrix during initialization.

% For the decoder module that generates segmentation masks, we gather information by concatenating temporal memory and sequential memory. The stride-16 feature map is projected to a single-channel logit via a 3 × 3 convolution and then bilinearly upsampled to the input resolution.

==> AnonymousSubmission/Writing/6_Experiments.tex <==
\section{Experiments}
\label{others}

% We demonstrate the effectiveness of our model and dataset through the video segment anything task and zero-shot transfer to video object segmentation task. Then, we ablate our model architecture and our inference methods.

\subsection{Datasets and evaluation}
In the training step, we first pre-train ViSAM on synthetic sequences by deforming static images to train the prompt generator stably. Subsequently, we train ViSAM on the ViSA dataset. Through this, ViSAM can learn the ability to segment and track the targets with various granularity. We also evaluate the performance of ViSAM on ViSA testset and compare it with existing SAM-based video segmentation methods. For this, we introduce video segment anything task. The objective of the video segment anything task is to segment the target track of the entire video clip from the provided prompts at the initial frame. Notably, the targets of video segment anything include not only foreground but also background, stuff, and part. Therefore, to achieve this, it is required the ability to segment targets of various types and granularity. Additionally, to validate the effectiveness of our framework on existing video task, we evaluate ViSAM on video object segmentation dataset~\cite{pont20172017} without training on the video object segmentation dataset.

To ensure the consistency of the annotated mask, we only leveraged mask tracks that exceed \(\mathrm{IoU}\) threshold  0.9 on every frame notated in equation \ref{iou_eq}. In this manner, mask tracks are generated by tracking the masks from the initial frame. In the final dataset, a mask track is included if its \(\mathrm{IoU}(\tilde{M}_{t-1}^i, \hat{M}_t^i)\) exceeds a threshold \(\gamma\) for all \(t\). We set \(\gamma\) to 0.9 for every experiments. We also collected and generated mask tracks from 174,025 video clips from HD-VILA-100M~\cite{xue2022hdvila}, 77,994 video clips remained after IoU filtering. Only filtered videos are used for training and evaluation. For the test, we randomly sampled 260 clips from ViSA dataset composed of 10 frames and the remaining 77,734 clips are used for training.
For evaluation, we use Jaccard Index $\mathcal{J}$,  boundary F1-score $(\mathcal{F})$, and the average of these $(\mathcal{J} \& \mathcal{F})$ in the video segment anything task and video object segmentation. In the video segment anything task, evaluation is performed independently for each individual mask, whereas in video object segmentation, evaluation is performed simultaneously for a frame.

\input{AnonymousSubmission/table/visa}

\subsection{Implementation details}
In this work, we use SAM pre-trained ViT-H~\cite{dosovitskiy2020image} as the image encoder. We freeze the image encoder, prompt encoder, and mask decoder excluding transformer block in the training step to preserve the capabilities of SAM. To train the transformer of SAM and our proposed prompt generator, we use one RTX 3090 GPU. We use short video clips of 6 frames for ViSA training. In both VOS and video segmentanything task, we use 8 points prompts per target and set $\alpha$ to 0.2. Through ablation studies we check the impact of these hyper parameters. The prompt generator consists of a two-layer standard transformer block that has single-head attention layers. The settings for the other modules, except for the prompt generator, follow~\cite{kirillov2023segment}. For optimization, we use AdamW~\cite{loshchilov2017decoupled} optimizer with a learning rate of 1e-5 and a weight decay of 0.05.
% mask decoder는 무슨 layer 몇개 쌓여있고 prompt generator는 무슨 layer 몇개 쌍요있고 mask decoder 뒤에는 무슨 upscaler가 달려있고 몇층짜리 mlp로 prompt 처리하고

\paragraph{Post Processing}
We improved the quality of the ViSAM output by post-processing it with SAM. The procedure began by selecting points from the binary mask produced by ViSAM. We utilized K-means clustering techniques to ensure an even distribution of sampled points across the mask. This method ensures that the sampled points cover the majority of the region, including different parts of the object, and it is robust against noise and outliers. In our zero-shot transfer experiments, we set the number of clusters to sample to 10.



\subsection{Main results}



\paragraph{Video segment anything task}
We evaluate existing video segmentation models~\cite{zou2024segment, zhou2024sam, zhang2023personalize, rajivc2023segment, cheng2022xmem, wang2023look, cheng2023tracking, oh2019video, wang2023images} that utilize the prompts such as mask, box, and points on our proposed ViSA dataset with ViSAM. For fair comparison, we use same hyper-parameter settings as in the zero-shot transfer to video object segmentation experiment and we retrain XMem, which has the highest performance in ViSA test set among exisiting methods, on the ViSA train set to compare it with ViSAM. Through this, we demonstrate that the existing video segmentation model can also acquire the capabilities to segment various types and granularities of targets via ViSA dataset, but the SAM-based video segmentation model can learn a more comprehensive knowledge of SAM. Table~\ref{Table:visa} shows the quantitative results. we also provide the qualitative results in the appendix.


\input{AnonymousSubmission/table/able_1}

\input{AnonymousSubmission/table/able_2}


\subsection{Ablation studies}

We conducted ablation studies on DAVIS-2017~\cite{pont20172017} about the type of prompts, datasets to train ViSAM, our inference method, and the number of point prompts per a track to confirm the effectiveness of our proposed module and dataset. Table~\ref{tab:abl_prompt_type},~\ref{tab:abl_training_data},~\ref{tab:abl_num_points}, and~\ref{tab:abl_sta} shows these results.

==> AnonymousSubmission/Writing/6_Experiments_new.tex <==
\section{Experiments}
\label{others}

% We demonstrate the effectiveness of our model and dataset through the video segment anything task and zero-shot transfer to video object segmentation task. Then, we ablate our model architecture and our inference methods.

\subsection{Evaluation metric}
% \subsection{Datasets and evaluation}
% In the training step, we first pre-train MMPM on synthetic sequences by deforming static images to train the prompt generator stably. Subsequently, we train MMPM on the ViSA dataset. Through this, MMPM can learn the ability to segment and track the targets with various granularity. We also evaluate the performance of MMPM on ViSA testset and compare it with existing SAM-based video segmentation methods. The objective of the video segment anything dataset is to segment the target track of the entire video clip from the provided segmentation mask at the initial frame. Notably, the targets of video segment anything include not only foreground but also background, stuff, and part. Therefore, to achieve this, it is required the ability to segment targets of various types and granularity. Additionally, to validate the effectiveness of our framework on existing video task, we evaluate MMPM on video object segmentation dataset~\cite{pont20172017} without training on the video object segmentation dataset.

For the evaluation metric, we use the Jaccard Index ($\mathcal{J}$), the boundary F1-score ($\mathcal{F}$), and the average of these metrics ($\mathcal{J} \& \mathcal{F}$) in the MUG-VOS dataset. In MUG-VOS, evaluation is performed independently for each individual mask, whereas in video object segmentation, evaluation is performed simultaneously across all masks in a frame.

\input{AnonymousSubmission/table/visa}

\subsection{MUG-VOS evaluation}
In order to evaluate the capability of multi-granularity segmentation in a video scene, we tested our models on the MUG-VOS dataset, which contains high-quality masks with a variety of granularities. To demonstrate that our MMPM model is best suited to the MUG-VOS dataset, we also tested the MUG-VOS dataset with other existing models~\cite{zhang2023personalize, rajivc2023segment, cheng2022xmem, cheng2023tracking}.
Specifically, since our MMPM leverages SAM's knowledge for video segmentation, we implemented a SAM-based baseline model that retrieves the mask proposal with the highest IoU score relative to the previous frame. Masks were initialized by providing grid points to SAM on every frame, and mask tracks were subsequently generated by sequentially selecting the mask with the highest IoU score.

Table~\ref{Table:visa} shows the quantitative results on MUG-VOS dataset.
For the SAM-based baseline, ``Grid" refers to the number of points per side when sampling points from the grid. The baseline demonstrated poor performance because it fails to generate the current frame's mask without relying on prior information from the previous frame. Additionally, solely relying on IoU for track connection makes it vulnerable to significant motion changes and occlusions.
While XMem and DEVA have shown great performance on the VOS task, they performed poorly on the MUG-VOS test set. Our experiments not only demonstrate that the MMPM model achieved the highest score compared to other models but also highlight that the MUG-VOS dataset is more challenging compared to existing VOS benchmarks. Previous VOS benchmarks only evaluate performance on salient objects, allowing models to be tuned to find the most prominent objects. However, to be effective in real-world settings, models should be capable of segmenting diverse object regardless of the spatial position of the target. 

Figure~\ref{fig:quality_comparision} shows the qualitative results compared with other methods. We will also provide more qualitative results in the appendix. MMPM demonstrated superior performance both quantitatively and qualitatively.

% \input{AnonymousSubmission/table/vos}

% \subsection{Video object segmentation}
% Although our MMPM model is trained to segment anything, we evaluated it on current VOS benchmarks in a zero-shot manner. We also compared it with existing state-of-the-art VOS models~\cite{zou2024segment, zhou2024sam, zhang2023personalize, rajivc2023segment, cheng2022xmem, wang2023look, cheng2023tracking, oh2019video, wang2023images}, as shown in Table~\ref{Table:vos}, using the same metrics we used to evaluate the ViSA dataset. For a fair comparison, we select existing video segmentation model that have best performance in ViSA test set and train it on ViSA training set.

% Although the MMPM model achieved the best performance on the ViSA dataset compared to other models, its performance slightly decreased when evaluated on other VOS benchmarks. This performance drop is because the MMPM model is not solely focused on prominent objects but also on non-salient objects, such as background elements and less noticeable items. While evaluating VOS performance on previous benchmarks is meaningful, it can be a misleading indicator since it only focuses on salient objects. We also provide the qualitative results on the previous VOS results in the appendix.

\input{AnonymousSubmission/table/able_1}
\input{AnonymousSubmission/table/able_2}

\subsection{Ablation study}
We conducted ablation studies on the MMPM model using the MUG-VOS test dataset. These studies explore the effects of different memory filtering methods, the number of memory values, memory update intervals, and the characteristics of each memory module.


Table~\ref{tab:memory_filtering_method} shows the performance of the MMPM model with different memory filtering methods. Firstly, no filtering is applied (i.e. Not filter) when memory reaches the limit $T_{max}$ and the memory retains the first inserted values for the entire video. Secondly, to append the latest values to memory, we implemented the First-In-First-Out (FIFO) method. Performance gain from FIFO method enables MMPM model to generate segmentation masks with the latest information enables the model to find corresponding objects efficiently. Thirdly, randomly filtering values from the memory allows the model to access diverse memories with random interval. Lastly, applying a constraint to the random filtering method to preserve the first and last frame values (i.e. P. first \& last), enhanced model performance compared to any other methods. Since, in VOS tasks, the initial mask from the first frame best represents the target object, and providing the latest mask to the MMPM model has a similar effect to the initial mask.

Table~\ref{tab:memory_type} shows the performance comparison between different memory usage types. To demonstrate the advantage of memory usage, we experimented with the MMPM model without memory values, where the mask is generated by referring only to the previous mask, indicated as `No memory'. Adding sequential memory, which is updated from selected frame, improved performance. The low-resolution sequential memory helps the model retrieve the target object. When temporal memory is added, the high-resolution information further enhances the model's ability to segment high-quality masks, as temporal memory stores diverse target information (e.g., shape, color, motion) from multiple frames.

Table~\ref{tab:memory_interval} shows the performance variation based on the interval period, denoted as \textit{r}, which determines when to update the memory. Increasing the interval between memory updates allows the model to perform faster inference while enabling it to store diverse information in memory. However, selecting an interval value that is too high can result in the loss of important intermediate information.

Table~\ref{tab:num_memory_value} shows the performance variation when implementing different number of memory values in the temporal memory, denoted as \textit{N}. Increasing number of value stored in temporal memory gave MMPM model to look over various memories. Abundant information from past frames enabled model to enhance to image embedding, resulting to MMPM to generate high quality segmentation mask. 
Interestingly, MMPM model performance has converged around the number of values 10. 

==> AnonymousSubmission/figure/latex/dataset_comparison_figure.tex <==
\begin{figure*}[ht]
    \centering
    % \vspace{-10pt}
    \includegraphics[width=\linewidth]{AnonymousSubmission/figure/MUG-VOS_comp.pdf}
    % \vspace{-10pt}
    \caption{\textbf{Comparison of granularities of video segmentation datasets:} Visualization of \textbf{(top)} MUG-VOS masks annotated by our data collection pipeline and ground-truth masks of Youtube-VOS~\cite{xu2018youtube}, DAVIS~\cite{pont20172017}, and UVO~\cite{wang2021unidentified} data and \textbf{(bottom)} MUG-VOS dataset. MUG-VOS masks include various types and granularities of objects, parts, stuff, and backgrounds, even those not covered by existing datasets.}
    % \vspace{-10pt}
    % \caption{\textbf{} Visualization of existing benchmarks mask annotations comparing ViSA mask quality.}
    \label{fig:dataset_comparison}
\end{figure*}

==> AnonymousSubmission/figure/latex/figure_main.tex <==
\begin{figure*}[t]
    \vspace{-10pt}
    \includegraphics[width=\linewidth]{AnonymousSubmission/figure/mmpm.pdf}
    \vspace{-15pt}
        \caption{\textbf{MMPM overview.} We introduce the MMPM model, which generates masks based on previous results. Starting from an initial mask that indicates the target object, the MMPM model consistently tracks and segments the target throughout the entire video. Sequential memory stores low-resolution features, updated at every selected frames, while temporal memory retains high-resolution features from previous frames, capturing a variety of information gathered from multiple frames.
        }
    \label{fig:overview}
    \vspace{-10pt}
\end{figure*}

% \begin{figure*}[t]
%     \begin{center}
%     \includegraphics[width=1\linewidth]{Figures/main_revised.pdf}
%     \end{center}
%     \vspace{-5pt}
%     \caption{\textbf{Overview.} \ours shows robust optimization of few-shot NeRF through MDE’s geometric prior, removing inherent ambiguity from MDE through novel patch-wise distillation loss and MDE adaptation.
%     Unlike existing work~\cite{uy2023scade} that distills depths by applying pretrained MDE to NeRF at seen view only, our \ours fully exploits the ability of MDE by jointly optimizing NeRF and MDE at a specific scene, and distilling the monocular depth prior to NeRF at both seen and unseen views.}
% \label{fig1:motivation}\vspace{-10pt}
% \end{figure*}

==> AnonymousSubmission/figure/latex/visa_engine_figure.tex <==
% \begin{figure*}[t]
%     \includegraphics[width=\linewidth]{figure/ViSAM_main.png}
%         \caption{\textbf{ViSAM overview.} We introduce the prompt generator to utilize SAM in the video domain. We also use frozen SAM image encoder and SAM mask decoder. We only train the transformer block of mask decoder and prompt generator to remain the knowledge of pre-trained SAM.
%         }
%     \label{fig:overview}
% \end{figure*}

\begin{figure*}[t]
    \vspace{-10pt}
    \includegraphics[width=\linewidth]{AnonymousSubmission/figure/data_engine.pdf}
    \vspace{-10pt}
        \caption{\textbf{MUG-VOS data collection pipeline.} We propose a data collection pipeline to generate a dataset to curate multi-granularity mask tracks completely automatically. Using SAM, we generate a large number of masks per frame and find a temporal connection through the IoU between the mask warped from the previous frame and the mask from the current frame.}
    \label{fig:engine}
    \vspace{-10pt}
\end{figure*}

==> AnonymousSubmission/table/able_1.tex <==
% \begin{table}[t]
% \centering
% \captionsetup{justification=centering}
% % \renewcommand{\arraystretch}{1.5}
% % \smaller[1]{
% \begin{subtable}[t]{0.50\linewidth}
%   \centering
%   \resizebox{\linewidth}{1.0cm}{ % Removed fixed height for better scaling
%     \begin{tabular}{l|ccc}
%       \toprule
%       Methods & $\mathcal{J\&F}$ & $\mathcal{J}$ & $\mathcal{F}$ \\
%       \midrule
%       Not filter & 85.0 & 85.7 & 84.2 \\
%       FIFO & 85.9 & 85.8 & 85.9 \\
%       Random & 86.0 & 85.9 & 86.0 \\
%       + Preserve first and last & 86.1 & 86.0 & 86.1 \\
%       \bottomrule
%     \end{tabular}
%   }
%   \caption{\textbf{Ablations on memory filtering methods.}}
%   \label{tab:memory_filtering_method}
% \end{subtable}
% % }
% \hfill
% % \renewcommand{\arraystretch}{1.13}
% % \smaller[1]{
% \begin{subtable}[t]{0.44\linewidth}
%   \centering
%   \resizebox{\linewidth}{1.0cm}{ % Removed fixed height for better scaling
%     \begin{tabular}{l|ccc}
%       \toprule
%       \textit{N} & $\mathcal{J\&F}$ & $\mathcal{J}$ & $\mathcal{F}$ \\
%       \midrule
%       5 & 85.7 & 85.8 & 85.5 \\
%       10 & 86.1 & 86.0 & 86.1 \\
%       15 & 86.1 & 86.0 & 86.1 \\
%       \bottomrule
%     \end{tabular}
% }   
%   \caption{\textbf{Ablations on number of temporal memory values.}}
%   \label{tab:num_memory_value}
% \end{subtable}
% % }
% \caption{Ablation studies on (a) memory filtering methods and (b) number of temporal memory values.}
% \label{tab:ablation_studies}
% \vspace{-10pt}
% \end{table}

\begin{table}[t]
\centering
\captionsetup{justification=centering}
\renewcommand{\arraystretch}{1.2} % Adjust row spacing for readability
\setlength{\tabcolsep}{3pt} % Adjust column spacing for a compact layout

\begin{subtable}[t]{0.48\linewidth} % Adjusted width for balance
  \centering
  \resizebox{\linewidth}{1.0cm}{ % Uniformly scale down the table
    \begin{tabular}{l|ccc}
      \toprule
      Methods & $\mathcal{J\&F}$ & $\mathcal{J}$ & $\mathcal{F}$ \\
      \midrule
      Not filter & 85.0 & 85.7 & 84.2 \\
      FIFO & 85.9 & 85.8 & 85.9 \\
      Random & 86.0 & 85.9 & 86.0 \\
      + P. first \& last & 86.1 & 86.0 & 86.1 \\
      \bottomrule
    \end{tabular}
  }
  \caption{\textbf{Memory filtering methods.}}
  \label{tab:memory_filtering_method}
\end{subtable}
\hfill
\begin{subtable}[t]{0.50\linewidth}
  \centering
  \resizebox{\linewidth}{1.0cm}{ % Fixed height
    \begin{tabular}{l|ccc}
      \toprule
      Methods & $\mathcal{J\&F}$ & $\mathcal{J}$ & $\mathcal{F}$ \\
      \toprule
      No memory & 81.8 & 85.3 & 78.2 \\
      + Only sequential & 81.9 & 85.3 & 78.5 \\
      + Only temporal & 85.7 & 85.9 & 85.8 \\
      + Both & 86.1 & 86.0 & 86.1 \\
      \bottomrule
    \end{tabular}
  }
  \caption{\textbf{Memory usage types.}}
  \label{tab:memory_type}
\end{subtable}


\caption{Ablation studies on (a) memory filtering methods and (b) number of temporal memory values.}
\label{tab:ablation_studies}
\vspace{-10pt}
\end{table}


==> AnonymousSubmission/table/able_2.tex <==
\begin{table}[t]
\centering
\captionsetup{justification=centering}
\smaller[1]{
\begin{subtable}[t]{0.44\linewidth}
  \centering
  \resizebox{\linewidth}{1.0cm}{ % Fixed height
    \begin{tabular}{l|ccc}
      \toprule
      \textit{r} & $\mathcal{J\&F}$ & $\mathcal{J}$ & $\mathcal{F}$ \\
      \toprule
      1 & 66.6 & 50.4 & 82.8 \\
      3 & 68.3 & 52.2 & 84.4 \\
      5 & 86.1 & 86.0 & 86.1 \\
      \bottomrule
    \end{tabular}
  }
  \caption{\textbf{Memory update interval.}}
  \label{tab:memory_interval}
\end{subtable}
}
\hfill
\begin{subtable}[t]{0.48\linewidth} % Ensure equal widths for balance
  \centering
  \resizebox{\linewidth}{1.0cm}{ % Uniformly scale down the table
    \begin{tabular}{l|ccc}
      \toprule
      \textit{N} & $\mathcal{J\&F}$ & $\mathcal{J}$ & $\mathcal{F}$ \\
      \midrule
      5 & 85.7 & 85.8 & 85.5 \\
      10 & 86.1 & 86.0 & 86.1 \\
      15 & 86.1 & 86.0 & 86.1 \\
      \bottomrule
    \end{tabular}
  }
  \caption{\textbf{Number of temporal memory values.}}
  \label{tab:num_memory_value}
\end{subtable}
\caption{Ablation studies on (a) memory update interval and (b) memory usage types.}
\label{tab:memory_ablation_studies}
\vspace{-10pt}
\end{table}

==> ArXiv/Writings/0_Abstract.tex <==
% \input{AnonymousSubmission/figure/latex/dataset_comparison_figure}

% \begin{abstract}
% Traditional video segmentation tasks are useful for segmenting clearly defined targets but have limitations in real-world applications such as interactive video editing where the target is not clearly defined. 
% \phseo{It is unclear to me what it means to be clearly defined. Are the objects in VOS clearly defined?}
% To tackle this issue, we introduce a new video segmentation task named video segment anything task that aims to segment any targets in the video data from provided prompts.
% \phseo{Maybe because of the previous statement, it is hard to accept that this task is new compared to VOS.}
% In this work, we aim to propagate the success of segment anything into the video domain, enabling its utilization in various real-world applications such as video understanding, editing, and processing. For this, we propose a large-scale densely annotated video segment anything (ViSA) dataset that includes various types and granularities of target annotations and a SAM-based data engine with an IoU-based tracking method to construct it. We also propose a simply designed baseline model, video segment anything model (ViSAM) to tackle the video segment anything task. As a result, ViSAM trained on ViSA dataset leads to the best performance on video segment anything task among the existing video object segmentation methods and SAM-based video segmentation methods. Additionally, we demonstrate the effectiveness of ViSA dataset and ViSAM through experiments on zero-shot transfer to video object segmentation. The project page with ViSA dataset and code will be made available soon.
% \end{abstract}


\begin{abstract}
Current benchmarks for video segmentation are limited to annotating only salient objects (i.e., foreground instances). Despite their impressive architectural designs, previous works trained on these benchmarks have struggled to adapt to real-world scenarios. Thus, developing a new video segmentation dataset aimed at tracking multi-granularity segmentation target in the video scene is necessary. In this work, we aim to generate multi-granularity video segmentation dataset that is annotated for both salient and non-salient masks.
% \phseo{The next sentences are not very well connected with the previous ones. It's like explaining the motivation from the start again.}
% In this work, we aim to propagate the success of the segment anything model ~\cite{kirillov2023segment} into the video domain, enabling its utilization in various real-world applications such as video understanding, editing, and processing. 
% \phseo{Maybe it's too late to discuss but is the name ``video segment anything'' good? I think there should be the term ``tracking'' instead of ``segmentation''.}
% For this, we propose a large-scale densely annotated video segment anything (ViSA) dataset that includes various types and granularities of target annotations. and a SAM-based~\cite{kirillov2023segment} data engine with an IoU-based tracking method to construct it. We also propose a baseline model, video segment anything model (ViSAM) to tackle the video segment anything task. 
To achieve this, we propose a large-scale, densely annotated multi-granularity video object segmentation (\textbf{MUG-VOS}) dataset that includes various types and granularities of mask annotations. We automatically collected a training set that assists in tracking both salient and non-salient objects, and we also curated a human-annotated test set for reliable evaluation.
% \phseo{What is the main contribution? the collection of the dataset itself? or the novel collection method?
% If it is the former, we may not include the method of generating the dataset in the abstract. Instead probably say that we colect a human-curated test set that can be used for reliable evaluation. Plus, we also collect a trainset automatically and show that it helps on tracking non-salient objects.}
In addition, we present memory-based mask propagation model (MMPM), trained and evaluated on MUG-VOS dataset, which leads to the best performance among the existing video object segmentation methods and Segment SAM-based video segmentation methods.
% Additionally, we demonstrate the effectiveness of ViSA dataset and ViSAM through experiments on zero-shot transfer to video object segmentation. 
Project page is available at \href{https://cvlab-kaist.github.io/MUG-VOS/}\texttt{https://cvlab-kaist.github.io/MUG-VOS/}.
\end{abstract}

==> ArXiv/table/data_stat.tex <==
\begin{table*}[t]
\centering
\begin{center}
\begin{tabular}{l @{\hspace{5mm}} c @{\hspace{5mm}} c @{\hspace{5mm}} c @{\hspace{5mm}} c @{\hspace{5mm}} c}
\toprule
 & Density & Masks & Mask Tracks & Masks per Frame & Annotated Frames \\
\midrule
OVIS~\cite{qi2022occluded} & 0.186 & 296k & 5,223 & 5.8 & 51,059 \\
YT-VIS~\cite{yang2019video} & 0.167 & 132K & 4,866 & 1.69 & 79,260 \\
YT-VOS~\cite{xu2018youtube} & 0.184 & 17K & 8,614 & 1.63 & 123,265 \\
DAVIS~\cite{pont20172017} & 0.120 & 27K & 386 & 2.6 & 150 \\
UVO~\cite{wang2021unidentified} & 0.425 & 593K & 104,898 & 12.3 & 58,140 \\
BURST~\cite{athar2023burst} & 0.167 & 600K & 16,089 & 3.1 & 195,713 \\
VIPSeg~\cite{Miao_2022_CVPR} & 0.979 & 926K & 38,592 & 10.9 & 3,536 \\
\midrule
\textbf{MUG-VOS Train} & 0.714 & 47M & 4.7M & 66.3 & 77,9940 \\
\textbf{MUG-VOS Test} & 0.663 & 59K & 887 & 29.6 & 1,999 \\
\bottomrule
\end{tabular}
\end{center}
\vspace{-5pt}
\caption{\textbf{Data comparison with previous video segmentation datasets.} Comparing MUG-VOS with existing video segmentation datasets in terms of statistics.}
\vspace{-10pt}
\label{Table:statistics}
\end{table*}


% https://yu-wu.net/pdf/CVPR22_VIPSeg.pdf#page=3.09
% https://arxiv.org/pdf/2209.12118 - BURST
% 

% \begin{table*}[t]
% \centering
% \begin{center}
% \begin{tabular}{l @{\hspace{5mm}} c @{\hspace{5mm}} c @{\hspace{5mm}} c @{\hspace{5mm}} c @{\hspace{5mm}} c}
% \toprule
% \textbf{Statistic} & Density & Masks & Mask Tracks & Masks per Frame & Number of video clips \\
% \midrule
% OVIS~\cite{qi2022occluded} & 0.186 & 131K & 4,883 & 5.9 & 607 \\
% YTVIS 2019~\cite{yang2019video} & 0.167 & 232K & 8,171 & 2.1 & 2,985 \\
% YTVIS 2021~\cite{yang2019video} & 0.167 & 296K & 5,223 & 2.1 & 2,985 \\
% DAVIS & 0.1204 & 32,875 & 448.5 & 2.99 & 150 \\
% UVO & 0.4257 & 132,732 & 14,748 & 12.29 & 11,361 \\
% BURST & & 600,157 & 16,089 & 3.0 & 2,914 \\
% VIPSeg & 0.9792 & 926K & 38753.6 & 10.9 & 3,536 \\
% \midrule
% \textbf{Ours} & \textbf{0.7140} & \textbf{47M} & \textbf{4.7M} & \textbf{66.3} & \textbf{70,977} \\
% \bottomrule
% \end{tabular}
% \end{center}
% \vspace{5pt}
% \caption{Comparing ViSA with OVIS~\cite{qi2022occluded} and YouTube-VIS~\cite{yang2019video} in terms of statistics.}
% \label{Table:statistics}
% \end{table*}











==> ArXiv/table/visa.tex <==
\begin{table*}[t]
\centering 
\begin{tabular}{lcccccc}
\toprule

MUG-VOS Test  &  & SAM & $\mathcal{J}\&\mathcal{F}$ & $\mathcal{J}$  & $\mathcal{F}$\\
\midrule
\textit{zero-shot transfer} & \\
SAM (Grid 32) + IoU & & $\tikzcmark$ & 22.2 & 20.2 & 24.2 \\
SAM (Grid 64) + IoU & & $\tikzcmark$ & 26.7 & 24.5 & 28.9 \\
PerSAM~\cite{zhang2023personalize} & & $\tikzcmark$ & 33.1 & 30.8 & 35.3 \\
PerSAM-F~\cite{zhang2023personalize} & & $\tikzcmark$ & 41.5 & 39.1 & 43.9 \\
SAM-PT~\cite{rajivc2023segment} &  & $\tikzcmark$ & 78.3 & 76.2 & 80.4 \\

\midrule

XMem*~\cite{cheng2022xmem} & & - & 83.0 & 86.9 & 79.1 \\
DEVA*~\cite{cheng2023tracking} &  & - & 85.6 & \underline{88.2} & 82.9 \\

\midrule
MMPM* & & - & \underline{86.1} & 86.0 & \underline{86.1} \\


\bottomrule
\end{tabular}
\caption{The quantitative evaluation on MUG-VOS test set. Note that * refers to a model trained on the MUG-VOS train set. ``SAM" correspond to an architecture that used SAM~\cite{kirillov2023segment} Encoder and Decoder.}
\vspace{-10pt}
\label{Table:visa}
\end{table*}


==> ArXiv/table/vos.tex <==
% \begin{table*}[t]
% \centering 
% \begin{tabular}{lcccccc}
% \toprule
%  & \multicolumn{3}{c}{Youtube-VOS} & \multicolumn{3}{c}{DAVIS-2017} \\
% \cmidrule(lr){2-4}
% \cmidrule(lr){5-7}
% &  $\mathcal{J}\&\mathcal{F}$ & $\mathcal{J}$ & $\mathcal{F}$ & $\mathcal{J}\&\mathcal{F}$ & $\mathcal{J}$  & $\mathcal{F}$\\
% \midrule
% STM~\cite{oh2019video} & 79.4 & \;-\; & \;-\; & \;81.8\; & \;79.2\; & \;84.3\; \\
% XMem~\cite{cheng2022xmem} & 86.1 & - &- &86.2 & 82.9 & 89.5 \\
% ISVOS~\cite{wang2023look} & 86.3 & - & - & 87.1 & 83.7 & 90.5 \\
% DEVA~\cite{cheng2023tracking} & - & - & - & 87.6 & 84.2 & 91.0 \\

% \midrule
% \textit{zero-shot transfer} & \\

% % Ours (+DV) & 77.8 & 79.1 & 83.5 &  70.8 & 77.8 \\
% Painter~\cite{wang2023images} & 24.1 & - & - &  34.6 & 28.5 & 40.8 \\
% SEEM~\cite{zou2024segment} & 53.8 & - & - &  62.8 & 59.5 & 66.2 \\
% SAM-PD~\cite{zhou2024sam} & 63.0 & - & - &  71.3 & 68.6 & 74.2 \\
% PerSAM~\cite{zhang2023personalize} & - & - & - &  66.9 & 71.3 & 75.1 \\
% PerSAM-F~\cite{zhang2023personalize} & 54.4 & - & - &  76.1 & 74.9 & 79.7 \\
% SAM-PT~\cite{rajivc2023segment} & 67.5 & - & - &  76.6 & 74.4 & 78.9 \\
% ViSAM & - & - & - &  75.3 & 72.9 & 77.7 \\

% \bottomrule
% \end{tabular}
%     \vspace{5pt}
% \caption{The quantitative evaluation of video object segmentation on Youtube-VOS~\cite{xu2018youtube} validation set and DAVIS-2017~\cite{pont20172017} validation set. Results for other methods are directly copied from~\cite{oh2019video, cheng2022xmem, wang2023look, zhou2024sam, cheng2023tracking}.}
% \label{Table:vos}
% \end{table*}


% \begin{table*}[t]
% \centering 
% \begin{tabular}{lccc}
% \toprule
%   & \multicolumn{3}{c}{DAVIS-2017} \\
% \cmidrule(lr){2-4}
% & $\mathcal{J}\&\mathcal{F}$ & $\mathcal{J}$  & $\mathcal{F}$\\
% \midrule
% STM~\cite{oh2019video} & \;81.8\; & \;79.2\; & \;84.3\; \\
% XMem~\cite{cheng2022xmem} &86.2 & 82.9 & 89.5 \\
% ISVOS~\cite{wang2023look} & 87.1 & 83.7 & 90.5 \\
% DEVA~\cite{cheng2023tracking} & 87.6 & 84.2 & 91.0 \\

% \midrule
% \textit{zero-shot transfer} & \\

% % Ours (+DV) & 77.8 & 79.1 & 83.5 &  70.8 & 77.8 \\
% Painter~\cite{wang2023images} &  34.6 & 28.5 & 40.8 \\
% SEEM~\cite{zou2024segment} &  62.8 & 59.5 & 66.2 \\
% SAM-PD~\cite{zhou2024sam} &  71.3 & 68.6 & 74.2 \\
% PerSAM~\cite{zhang2023personalize} &  66.9 & 71.3 & 75.1 \\
% PerSAM-F~\cite{zhang2023personalize} &  76.1 & 74.9 & 79.7 \\
% SAM-PT~\cite{rajivc2023segment} &  76.6 & 74.4 & 78.9 \\
% % ViSAM &  - & - & - \\
% \midrule
% ViSAM* & 69.1 & 66.0 & 72.1 \\

% \bottomrule
% \end{tabular}
%     \vspace{0pt}
% \caption{The quantitative evaluation of video object segmentation on DAVIS-2017~\cite{pont20172017} validation set. Results for other methods are directly copied from~\cite{oh2019video, cheng2022xmem, wang2023look, zhou2024sam, cheng2023tracking}. Note that * refers a model fine-tuned on the YouTube-VOS dataset.}
% \label{Table:vos}
% \end{table*}

\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{ % Scale the table to fit the text width
\begin{tabular}{lccccc}
\toprule
DAVIS-2017 & $\mathcal{J}\&\mathcal{F}$ & $\mathcal{J}$  & $\mathcal{F}$ \\
\midrule
XMem*~\cite{cheng2022xmem}  & 63.0 & 59.7 & 66.4 \\
DEVA*~\cite{cheng2023tracking}  & 64.1 & 60.8 & 67.4 \\
MMPM*  & \underline{69.1} & \underline{66.0} & \underline{72.1} \\
\bottomrule
\end{tabular}
}
\caption{The quantitative evaluation of video object segmentation on DAVIS-2017~\cite{pont20172017} validation set. Note that * refers to a model trained on the MUG-VOS train set.}
\vspace{-10pt}
\label{Table:vos}
\end{table}


